How to Configure Good In-Context Sequence for Visual Question Answering

Inspired by the success of Large Language Models in dealing with new tasks via In-Context Learning (ICL) in NLP, researchers have also developed Large Vision-Language Models (LVLMs) with ICL capabilities. However, when implementing ICL using these LVLMs, researchers usually resort to the simplest way like random sampling to configure the in-context sequence, thus leading to sub-optimal results. To enhance the ICL performance, in this study, we use Visual Question Answering (VQA) as case study to explore diverse in-context configurations to find the powerful ones. Additionally, through observing the changes of the LVLM outputs by altering the in-context sequence, we gain insights into the inner properties of LVLMs, improving our understanding of them. Specifically, to explore in-context configurations, we design diverse retrieval methods and employ different strategies to manipulate the retrieved demonstrations. Through exhaustive experiments on three VQA datasets: VQAv2, VizWiz, and OK-VQA, we uncover three important inner properties of the applied LVLM and demonstrate which strategies can consistently improve the ICL VQA performance. Our code is provided in: https://github.com/GaryJiajia/OFv2_ICL_VQA.

==> sec/7_material.tex <==
\clearpage
\setcounter{page}{1}
\twocolumn[{
\renewcommand\twocolumn[1][]{#1}
\maketitlesupplementary
\begin{center}
  \centering
  \includegraphics[width=17cm]{figure/Appendix_STI.pdf}
  \captionof{figure}{The schematic representation of more demonstrations retrieval strategies. (a) is Retrieving via Similar Image (SI) mentioned in Sec.3.2 in the main text of the paper, (b)-(f) is the image retrieval method mentioned in \cref{asec:retrieve_images}. Here we explore more specific retrieval methods, such as focusing on diversity in image retrieval ((c), (d)) and using another modality of information (text) for image retrieval ((e), (f)). }
  \label{fig:a_sti}  
\end{center}
}]
  
\section{More Demonstrations Retrieval Methods}
\label{asec:more_methods}
\subsection{Retrieving Images}
\label{asec:retrieve_images}
Here we introduce more methods centered around retrieving images from $\mathcal{D}$, subsequently using the corresponding triplet as the demonstrations.

\noindent\textbf{(1) Retrieving via Similar Tags from Image (STI)} (\cref{fig:a_sti} (b)).
We employ Vinvl \cite{zhang2021vinvl} and IETrans \cite{zhang2022fine} to extract three categories of tags (object, attribute, and relation) from the images in $\mathcal{D}$ and a given query image. Subsequently, we compute tag overlap between them, aiming to identify and return images from $\mathcal{D}$ exhibiting the highest similarity to the query. Consider a query image tagged with three tags:``dog", ``white" ,``drink". Suppose image A is tagged with ``cat", ``white", ``sit", and image B with ``dog", ``brown", ``drink". STI would prioritize image B due to its higher tag overlap, having two matching tags with the query image. In order to efficiently calculate the overlap in tags, we list all discrete tags utilizing a one-hot manner and then apply an ``AND" operation to assess the similarity at the tag level.

\noindent\textbf{(2) Retrieving via Diverse Image (DI).}
Some works in NLP have discovered that diverse demonstrations containing more relevant information can significantly enhance performance. Drawing on this insight, we retrieve images from $\mathcal{D}$ based on diversity. We extract specific semantic labels from the images and apply two partitioning methods to divide the semantic labels into different clusters to meet the diversity of images for each cluster: \textbf{1) Retrieving via Diverse Tags from Image (DT-I)} (\cref{fig:a_sti} (c)): we first extract three categories of tags (object, attribute, and relation) from $\hat{\bm{I}}$. Suppose there are total $m$ kinds of tags, we divide them into $n$ clusters and there are $m/n$ kinds of tags in each cluster. Within each tag cluster, only the tags in that specific cluster are used to calculate the similarity score between two images, which is based on the number of tags both images share, using the SI method. \textbf{2) Retrieving via Diverse Categories from Image (DC-I)} (\cref{fig:a_sti} (d)): we extract four categories of tags (object, attribute, relation, and class) from the images and categorize the tags into four respective clusters. For example, one cluster will solely contain object tags, while another may only encompass relation tags. This categorization process allows for a more holistic capture of all four content dimensions, retrieving the top-$\bm{n/4}$ similar images within each clusters.

\begin{figure*}[t]
  \centering
  \includegraphics[width=17.5cm]{figure/SM_example_cases2.pdf}
  \caption{Some Example input-output samples from our experiment of Open-Flamingo.}
  \label{fig:sm_example_cases}
\end{figure*}


% % ground truth 还是 ground-truth
\noindent\textbf{(3) Retrieving Image via Similar Text.} 
In addition to using $\hat{\bm{I}}$ to retrieve images from $\mathcal{D}$, retrieving images based on the query text represents a method that can more effectively leverage the correlation between the visual modality and the linguistic modality. Considering that the image encoder and text encoder of CLIP can respectively map images and text into an embedding space, we employ the CLIP embedding of the query text to retrieve the corresponding embedding of images from $\mathcal{D}$. We propose two methods for text-based image retrieval: \textbf{1) Retrieving Image via Similar Question (I-SQ)} (\cref{fig:a_sti} (e)): we evaluate the similarity between the CLIP embedding of the query question $\hat{\bm{Q}}$ and the CLIP embedding of each image ${\bm{I}}$ in $\mathcal{D}$. \textbf{2) Retrieving Image via Similar Question\&Answer (I-SQA)} (\cref{fig:a_sti} (f)): we use the CLIP embedding of the combination of $\hat{\bm{Q}}$ and the ground truth answer to retrieve images from $\mathcal{D}$ based on similarity metrics.


\subsection{Retrieving Questions and Answers}
\noindent\textbf{(1) Retrieving via Similar Tags from Question (STQ).} We extract different categories of tags from questions. Rather than leveraging the entire question sentence, we select pivotal tags for similarity retrieval. We adopt two types of settings: 1) Use the two most essential tags \textbf{(STQ-2)}: objects and relations. 2) Use four categories of tags \textbf{(STQ-4)}: objects, relations, attributes and interrogative words. Interrogative words are used to identify the type of questions, like ``When".

\noindent\textbf{(2) Retrieving via Diverse Question (DQ).} Similar to DI, more diverse demonstrations enhance the comprehension and reasoning capabilities of the model. In addition to the vision level of diversity retrieval, we also perform diversity retrieval at the language level. We extract four categories of tags from questions: objects, relations, attributes and interrogative words. And we employ STQ to obtain the top-$\bm{n/4}$ similar questions within each category. 


\noindent\textbf{(3) Retrieving Text via Similar Image.}
Similar to I-SQ and I-SQA, in addition to using text to retrieve questions from $\mathcal{D}$, we also use images to retrieve text, aiming to combine information from both visual and linguistic modalities. Specifically, we use  $\hat{\bm{I}}$ to retrieve two types of text from $\mathcal{D}$: \textbf{1) Retrieving Question via Similar Image (Q-SI)}: we use the CLIP embedding of $\hat{\bm{I}}$ to retrieve the questions from $\mathcal{D}$. \textbf{2) Retrieving Question\&Answer via Similar Image (QA-SI)}: we use the CLIP embedding of $\hat{\bm{I}}$ to retrieve the question-answer pairs $\{(\bm{Q}_1,\bm{A}_1);(\bm{Q}_2,\bm{A}_2);...;(\bm{Q}_n,\bm{A}_n)\}$ from $\mathcal{D}$.

\subsection{Manipulating Demonstrations}
\noindent\textbf{(1) Changing the Orders of Demonstrations}. 
Some works in NLP have discovered the orders of the demonstrations  can impact performance. Consequently, we also experiment with reversing the order of the demonstrations. We invert the original in-context sequence $\mathcal{S}$ to $\mathcal{S'}=\{(\bm{I}_n,\bm{Q}_n,\bm{A}_n);...;
(\bm{I}_2,\bm{Q}_2,\bm{A}_2)
(\bm{I}_1,\bm{Q}_1,\bm{A}_1);
(\hat{\bm{I}},\hat{\bm{Q}})\}$.


\noindent\textbf{(2) Changing Question-Answer Pairs into Declarative Sentences}. 
Some works like \cite{liu2022declaration} manipulate question-answer pairs into declarative sentences to better adapt to the pre-training language model. We follow \cite{liu2022declaration} to manipulate the question-answer pairs, in which the corresponding short answer is replaced with a [MASK] token. For example, the question ``How many animals are there?" can be changed into ``There are [MASK] animals". Then we add the declarative sentences into the in-context sequence $\mathcal{S'}=\{(\bm{I}_1,\bm{D}_1,\bm{A}_1);...;(\bm{I}_n,\bm{D}_n,\bm{A}_n);(\hat{\bm{I}},\hat{\bm{D}})\}$, where $\bm{D}$ denotes the declarative sentence.

% \noindent\textbf{Ensemble Retrieval Method}.
% %ensemble
% Considering the diverse nature of questions, \eg, seeking information on time, location, requiring binary responses, we adopt an ensemble retrieval strategy approach for optimal in-context learning. Instead of relying on a universal method for all questions, our ensemble approach categorizes each incoming question into one of the predefined categories. After classifying, it utilizes the most suitable retrieval strategy tailored for that specific question category.


\begin{figure*}[t]
  \centering
  \includegraphics[width=17cm]{figure/SM2_TRTLexper2.pdf}
  \caption{The experiments on disentangling TR and TL. Three settings are conducted: (1) ``Standard" provides the correct demonstrations. (2) ``Mismatch" randomly replaces answers to evaluate TR capability. (3) ``New mapping" substitutes ``yes/no" with novel answers to test TL capability.}
  \label{fig:sm_experiment_trtl}
\end{figure*}


\section{Experiments}
\subsection{More Details about Datasets and Evaluation Metric}
\noindent\textbf{VQAv2.}
VQAv2~\cite{goyal2017vqav2} is a widely-used benchmark for visual question answering, consisting of 443,757 training and 214,354 validation questions. The dataset includes general images sourced from the MSCOCO dataset. Each image is associated with multiple questions and human-annotated answers, reflecting a combination of high-quality visual and commonly encountered questions.

\noindent\textbf{VizWiz.}
The VizWiz dataset~\cite{bigham2010vizwiz} is dedicated to answering visual questions from individuals who are blind. It consists of 20,523 training image/question pairs and 4,319 validation image/question pairs. Blind participants captured images and asked spoken questions, with 10 crowd-sourced answers per question. Due to this, the VizWiz dataset exhibits low-quality images and questions, also with a significant number of unanswerable questions.

\noindent\textbf{OK-VQA.}
OK-VQA~\cite{marino2019okvqa} aims to challenge models to leverage external knowledge for accurate answers. The dataset comprises 14,055 open-ended questions, each associated with five ground truth answers. All questions have been carefully filtered to ensure they necessitate external knowledge, such as information from Wikipedia.

\noindent\textbf{Evaluation Metric.} We follow \cite{alayrac2022flamingo} to use accuracy as the evaluation metric for VQA task. The detailed calculation formula is as follows:
\begin{equation} \label{equ:acc}
    Acc_{a_i} = max(1,\frac{3\times \sum_{k\in [0,9]}^{} match(a_i,g_k)}{10}),
\end{equation}
where $a_i$ denotes the predicted answer of the LVLM, $g_k$ denotes the $k$-th ground true answer, and the $match()$ function indicates whether two answers match, if they match, the result is 1, otherwise it is 0.

\subsection{Implementation Details of Auxiliary Experiments}
\noindent\textbf{Disentangling TR and TL Following ~\cite{tr&tl}.}
We conduct experiments on disentangling TR and TL following ~\cite{tr&tl} as shown in \cref{fig:sm_experiment_trtl}. Specifically, we use different demonstration settings to reflect the TR and TL capabilities of models. We employ the standard in-context learning setting (\textbf{``standard"}) to represent the overall ICL (In-Context Learning) ability of the model, which involves the simultaneous application of TR and TL. Additionally, we use the Mismatching Answer (MA) method (\textbf{``mismatch"}), where the answers in the demonstrations are replaced with random answers that are 50\% correct and 50\% incorrect. This experiment aims to assess the TR ability of model, as format TR only requires the answer space to match the correct answer, while the mapping of incorrect answers significantly affects TL performance. Furthermore, we replace the answer in the demonstrations with an answer from a different answer space, forming a new mapping relationship (\textbf{``new-mapping"}). For example, replacing ``yes" with ``tiger" and ``no" with ``lion". This experiment aims to evaluate the TL ability of model, as such mapping relationships are rarely encountered during pre-training. To facilitate the replacement of the answer space, this experiment is conducted using only the ``yes/no" type questions from the VQAv2 dataset.

\begin{figure*}[t]
  \centering
  \includegraphics[width=17.5cm]{figure/SM3_noisycase2.pdf}
  \caption{The samples of the experiments on adding noise to the query image. (a) showcases a scenario where demonstrations are randomly sampled and no noise is added to the query image. The model correctly identifies the room as a ``playroom" in response to the question. (b) depicts the use of identical demonstrations but with the query image blurred. The blurred image is difficult to provide effective visual information, resulting in incorrect answers. This error may be influenced by the second demonstration, which erroneously suggests a ``bathroom" scene. (c) employs image similarity for demonstrations retrieval and blurs the query image. However, the demonstrations in this instance provide relevant visual information, enabling the model to identify that this is in a ``computer room".   }
  \label{fig:sm_experiment_noisy}
\end{figure*}


\noindent\textbf{Adding Noise to the Query Image and Question.} 
To better compare the roles of visual information and textual information in TR, we conduct experiments adding noise to the query image and question, effectively diminishing the presence of pertinent information. Specifically, as shown in \cref{fig:sm_experiment_noisy}, we design two distinct experiments: \textbf{1) Adding Noise to the Image}: we apply Gaussian blur to the query image to blur the inherent visual information. As shown in \cref{fig:sm_experiment_noisy} (b) and (c), the noise results in a loss of visual information, leading to errors in answers, while SI method can partially compensate for the loss of visual information. Although the answer is still incorrect in Figure 3 (c), the additional image information enables the model to acknowledge the potential presence of visual elements such as the ``computer" in the original image, which can compensate for the visual TR ability to some extent. \textbf{2) Adding Noise to the Question}: we manipulate the query question by filtering out key information, such as nouns in the question which generally represent the object to be asked. Removing the key information may potentially hinder the model to understand what is being asked.


\subsection{Implementation Details of Preparing Instructions}
To better guide the generation of answers by LVLM, we attempt to add instructions to the input information. Besides using instructions written by humans, we also utilize instructions prompted by GPT-4 to further guide the LVLM. Considering that the VQA task on the OK-VQA dataset relies on external knowledge to answer questions, appropriate instructions might better stimulate the TL capability of the model. Therefore, our primary focus is to explore the impact of diverse instructions on performance for the OK-VQA dataset. Beyond manually written instructions, we have employed plowerful LLM, GPT4\cite{openai2023gpt}, to generate instructions. Specifically, we input our task description and instruction requirements to GPT4, asking it to output various instructions. We mainly require it to generate concise, straightforward instructions and detailed, hierarchical instructions. \cref{fig:sm_prompt_by_gpt4} displays the prompts we use and the responses from GPT-4.

\begin{table*}[htb]
  \centering
  \scalebox{0.8}{
  \setlength{\tabcolsep}{4mm}{
  \begin{tabular}{@{}lcccccc@{}}
  \toprule
          & \multicolumn{3}{c}{OFv1}  & \multicolumn{3}{c}{OFv2}  \\ 
            \cmidrule(r){2-4}  \cmidrule(r){5-7}
       & 4-shot & 8-shot & 16-shot 
       & 4-shot & 8-shot & 16-shot\\
    \midrule
    RS       
    & 44.56  & 47.38  & 48.71   
    & 48.82  & 51.05  & 50.89   \\
    \midrule
    STI
    & 44.61  & 47.89  & 49.91
    & 50.02  & 51.83  & 51.89   \\
    I-SQ      
    & 44.22  & 47.18  & 49.29   
    & 47.14  & 50.47  & 50.96   \\
    I-SQA     
    & 43.84  & 46.58  & 48.31   
    & 47.20  & 48.43  & 49.29   \\
    \midrule
    STQ-2     
    & 48.58  & 50.01  & 51.47   
    & 47.53  & 49.28  & 49.42   \\
    STQ-4     
    & 49.74  & 51.16  & 52.58   
    & 48.69  & 50.18  & 48.83   \\
    Q-SI    
    & 43.07  & 45.56  & 47.33   
    & 46.54  & 49.12  & 48.56   \\
    QA-SI     
    & 45.24  & 47.83  & 49.14   
    & 47.52  & 49.65  & 50.28   \\
    \bottomrule
  \end{tabular}}
  }
  \caption{Experimental Results on the VQAv2 Dataset for more \textbf{Similarity-based Methods} in 4-shot, 8-shot, and 16-shot Learning Settings.}
  \label{table:more_similarity}
\end{table*}

\begin{table*}[htb]
  \centering
  \scalebox{0.8}{
  \setlength{\tabcolsep}{4mm}{
  \begin{tabular}{@{}lcccccc@{}}
  \toprule
          & \multicolumn{3}{c}{OFv1}  & \multicolumn{3}{c}{OFv2}  \\ 
            \cmidrule(r){2-4}  \cmidrule(r){5-7}
       & 4-shot & 8-shot & 16-shot 
       & 4-shot & 8-shot & 16-shot\\
    \midrule
    RS       
    & 44.56  & 47.38  & 48.71   
    & 48.82  & 51.05  & 50.89   \\
    \midrule
    DT-I
    & 46.44  & 48.18  & 49.86
    & 49.27  & 51.75  & 51.09   \\
    DC-I
    & 45.97  & 48.52  & 49.86
    & 48.98  & 51.59  & 50.61   \\
    \midrule
    DQ     
    & 47.03  & 49.24  & 50.24   
    & 49.84  & 51.09  & 49.99   \\
    \bottomrule
  \end{tabular}}
  }
  \caption{Experimental Results on the VQAv2 Dataset for \textbf{Diversity-based Methods} in 4-shot, 8-shot, and 16-shot Learning Settings.}
  \label{table:diversity}
\end{table*}

\begin{table}[htb]
  \centering
  \scalebox{0.8}{
  \setlength{\tabcolsep}{2mm}{
  \begin{tabular}{@{}lcccccc@{}}
  \toprule
          & \multicolumn{3}{c}{OFv1}  & \multicolumn{3}{c}{OFv2}  \\ 
            \cmidrule(r){2-4}  \cmidrule(r){5-7}
       & 4-shot & 8-shot & 16-shot 
       & 4-shot & 8-shot & 16-shot\\
    \midrule
    RS       
    & 44.56  & 47.38  & 48.71   
    & 48.82  & 51.05  & 50.89   \\
    \midrule
    SI        
    & 47.30  & 49.65  & 51.70
    & 50.36  & 52.95  & 54.1   \\
    SI + Reverse 
    & 47.10  & 49.74  & 51.59
    & 50.54  & 53.23  & 53.84   \\
    \midrule
    SQ        
    & 48.82  & 50.84  & 51.88   
    & 47.49  & 50.16  & 49.16   \\
    SQ + Reverse
    & 47.75  & 49.79  & 50.80
    & 47.38  & 48.77  & 47.74   \\
    \bottomrule
  \end{tabular}}
  }
  \caption{Experimental Results on the VQAv2 Dataset for \textbf{reversing the Order of Demonstrations} in 4-shot, 8-shot, and 16-shot Learning Settings.}
  \label{table:reverse}
\end{table}

\begin{figure}[t]
  \centering
  \includegraphics[width=8cm]{figure/SM4_instruct3.pdf}
  \caption{Scenario of using GPT4 for instructions generation . We first use concise language to describe our task, and then inform GPT4 of our requirements.}
  \label{fig:sm_prompt_by_gpt4}
\end{figure}


\section{More Experimental Results}
% Here we present all the numerical results from the experiment in \cref{table:vqav2_all_experiments}, based on different demonstrations retrieval and manipulate method. 

Here, we present all the numerical results from the experiments, which are based on different demonstration retrieval and manipulation methods that are not mentioned in the main text. These methods are not discussed in the main text because they do not show significant improvement in the performance of OF or exhibit unstable results.


\cref{table:more_similarity} showcases more similarity-based retrieval methods, including tag-based retrieval, which yields similar results to the embedding-based retrieval method mentioned in the main text. Both approaches exhibit stable improvements. However, using mixed modality for retrieval (I-SQ, I-SQA, Q-SI, and QA-SI) does not provide significant assistance to the performance of model and may even lead to performance degradation. This could be attributed to the limited amount of image-related information present in the questions. Consequently, using images to retrieve questions or using questions to retrieve images is not a viable choice.

\cref{table:diversity} displays the results of using diversity-based retrieval methods. It can be observed that enhancing the diversity of similar demonstrations can improve the results to some extent, but compared to similarity retrieval, it cannot yield significant improvements for OF.


\begin{table}[t]
  \centering
  \scalebox{0.8}{
  \setlength{\tabcolsep}{3mm}{
  \begin{tabular}{@{}lccc@{}}
  \toprule
    & 4-shot & 8-shot & 16-shot\\
    
    \midrule
    RS       
    & 48.82  & 51.05  & 50.89   \\
    RS + Declarative Sentences       
    & 33.19  & 38.61  & 39.21   \\
    \midrule
    SI*        
    & 51.23  & 52.14  & 52.55   \\
    SI* + Declarative Sentences
    & 41.89  & 44.04  & 44.11   \\
    \bottomrule
  \end{tabular}}
  }
  \caption{Experimental Results on the VQAv2 Dataset for \textbf{changing Question-Answer Pairs into Declarative Sentences} in 4-shot, 8-shot, and 16-shot Learning Settings. SI* denotes that we use SI to retrieve images and limit the retrieved images to be non repetitive.}
  \label{table:declaration}
\end{table}

\begin{table*}[h]
  \centering
  \renewcommand\arraystretch{1.3}
  \tabcolsep=3mm
  \scalebox{0.8}{
  \begin{tabular}{@{}p{10cm}  c c c@{}}
    \toprule
    Instruction  & 4 shot & 8 shot &   16 shot \\
    \midrule
    RS
    & 34.82 & 38.54 & 39.55 \\
    
    According to the previous question and answer pair, answer the final question.
    & 35.72 & 39.38 & 40.46 \\

    Using external knowledge and image content to answer questions.
    & 34.28 & \textbf{40.47} & 40.69 \\

    Integrate information from the question, image, and previous answers.
    & 36.40 & 40.46 & 40.88 \\

    Consider the semantic relationship between the question and the image.
    & \textbf{36.45} & 40.17 & \textbf{41.11} \\

    For the upcoming tasks, you'll be provided image-text pairs. Digest these pairs carefully. Later, an image along with a question will be presented. Combine your understanding from the pairs, the new image, and your own knowledge to answer.
    & 35.13 & 40.30 & 40.61 \\
    
    You will be engaged in a two-phase task. Phase 1: Absorb the information from a series of image-text pairs. Phase 2: Use that context, combined with an upcoming image and your own database of knowledge, to accurately answer a subsequent question.
    & 35.53 & 40.19 & 40.02 \\
    \bottomrule
  \end{tabular}
  }
  \caption{Experimental Results of RS on the VQAv2 Dataset for \textbf{using different instructions} in 4-shot, 8-shot, and 16-shot Learning Settings.}
  \label{table:instruction_sm}
\end{table*}


\begin{table*}[t]
  \centering
  \scalebox{0.8}{
  \setlength{\tabcolsep}{4mm}{
  \begin{tabular}{@{}lllcccc@{}}
  \toprule
      & LVLM & Language Model & 4-shot & 8-shot & 16-shot & Average \\
    \midrule
    RS & Open-Flamingo & LLAMA-7B      
    & 44.56  & 47.38  & 48.71 & 46.88 \\
    RS & Open-Flamingo & MPT-7B   
    & 48.82  & 51.05  & 50.89 & 50.25 \\
    RS & Otter & LLAMA-7B      
    & 39.14  & 41.28  & 42.43 & 41.13 \\
    RS & Otter & MPT-7B   
    & 24.96  & 27.60  & 29.92 & 27.49 \\
    \midrule
    SI & Open-Flamingo & LLAMA-7B       
    & 47.30  & 49.65  & 51.70 & 49.55 \\ 
    SI & Open-Flamingo & MPT-7B
    & 50.36  & 52.95  & 54.10  & 52.47 \\
    SI & Otter & LLAMA-7B      
    & 37.61  & 39.72  & 41.42 & 39.58 \\
    SI & Otter & MPT-7B      
    & 23.08  & 24.38  & 23.95 & 23.80 \\
    \midrule
    SQ & Open-Flamingo & LLAMA-7B       
    & 48.82  & 50.84  & 51.88 & 50.82 \\
    SQ & Open-Flamingo & MPT-7B
    & 47.49  & 50.16  & 49.16 & 48.94 \\
    SQ & Otter & LLAMA-7B      
    & 39.16  & 39.41  & 40.57 & 39.71 \\
    SQ & Otter & MPT-7B      
    & 23.29  & 23.56  & 22.74 & 23.20 \\
    \bottomrule
  \end{tabular}}
  }
  \caption{Experimental Results on the \textbf{different Large Vision-Language Models} in 4-shot, 8-shot, and 16-shot Learning Settings.}
  \label{table:different_models}
\end{table*}

\cref{table:reverse} presents the impact of inputting similar demonstrations in reverse order to the model. Previous studies in the field of NLP~\cite{liu2021selection} have found that placing more similar samples closer to the query can lead to greater performance improvements. However, based on the experimental results in this paper, such manipulation has little effect on OF.

\cref{table:declaration} illustrates the effect of changing questions into declarative sentences. This transformation evidently leads to a marked reduction in performance of the model. One potential explanation for this phenomenon could be the difficulty for the model in recognizing the [mask] token. This challenge hinders the model to grasp the underlying reasoning requirements in the task. Consequently, this approach does not yield a significant improvement in OF either.

\cref{table:instruction_sm} presents the outcomes of offering different instructions. Both the concise instructions and the detailed, hierarchical instructions result in noticeable enhancements compared to the Random Sampling (RS) outcomes. Notably, concise and pertinent instructions appear to yield superior results. Building on these findings, we plan to delve deeper into the efficacy of different instructional methodologies.
% \cref{table:more_instruct_mismatch} ?

% \noindent\textbf{Changing the Orders of Demonstrations}. 

% \noindent\textbf{Changing Question-Answer Pairs into Declarative Sentences}. 

% \noindent\textbf{More Results of instructions and mismatch}.



\section{Experiments on More Large Vision-Language Models}
In our study, we primarily utilized Open-Flamingo, a Large Vision-Language Model (LVLM), as our experimental model. Additionally, we also explored other LVLMs that support in-context learning. For instance, we examine Otter\cite{li2023otter}, a LVLM based on Open-Flamingo, is fine-tuned on the MIMIC-IT multimodal dataset\cite{li2023mimic} for enhancing performance.

Furthermore, We compare the performance of these models trained on different large language models (LLMs). The primary distinction between Otter v1 and Otter v2 lies in their language models, similar to Open-Flamingo, Otter v1 utilizes LLAMA-7B, while Otter v2 employs MPT-7B. The outcomes of these comparative experiments are shown in \cref{table:different_models}.

==> sec/experiment_temp.tex <==
\section{Experiments}

\subsection{Datasets and Implementation Details}
%dataset介绍这里，一定要写出这个vqa场景的特色，比如vqav2是比较标准的从图片里根据question来回答，但是vizwiz的话要强调图像质量不行，回答的质量也不行，至少不标准，okvqa要强调要额外的knowledge，需要commonsense
\noindent\textbf{VQAv2.}
VQAv2 is a widely-used benchmark for visual question answering, consisting of 443,757 training and 214,354 validation questions. The dataset includes general images sourced from the MSCOCO dataset. Each image is associated with multiple questions and human-annotated answers, reflecting a combination of high-quality visual and commonly encountered questions.

\noindent\textbf{VizWiz.}
%数据集的名称不能错，大小写查清楚，这里只是我随手写的
The VizWiz dataset is dedicated to answering visual questions from individuals who are blind. It consists of 20,523 training image/question pairs and 4,319 validation image/question pairs. Blind participants captured images and asked spoken questions, with 10 crowdsourced answers per question. Due to this, the VizWiz dataset exhibits low-quality images and questions, also with a significant number of unanswerable questions.

\noindent\textbf{OKVQA.}
OKVQA aims to challenge models to leverage external knowledge for accurate answers. The dataset comprises 14,055 open-ended questions, each associated with five ground truth answers. All questions have been carefully filtered to ensure they necessitate external knowledge, such as information from Wikipedia.

\noindent\textbf{Implementation Details}
We employ the Open-Flamingo v1 and v2 as the LVLM to evaluate the strategies of demonstration configurations. During retriving, to calculate the embedding similarity, we use the ViT-B/32 model as the vision encoder and a 12-layer Transformer from a well-trained CLIP model as the language encoder to extract image and sentence embeddings. In ICL, we use 4, 8, 16, and 32-shots demonstrations. All experiments are conducted on a single RTX 3090 GPU, utilizing FP16 precision.

\begin{figure*}[htb]
  \centering
  \includegraphics[width=15cm]{figure/trtl-more3.pdf}
  \caption{Impact of different demonstration configuration strategies on model performance: Insights from task recognition and task learning perspectives.}
  \label{fig:more_trtl}
  % \vspace{-0.2in}
\end{figure*}

\subsection{Results and Analyses}
Since exhaustive retrieval and manipulation techniques are applied to configure in-context sequence, presenting all these experimental results could lead to disarray. To avoid confusions and emphasize the major conclusions, we show the corresponding experiment results of each claim in the following and list all the results in the Supplementary Material. Next, in Section~\ref{sec 4.1}, we first show the characteristics of the applied LVLM, Open-Flamingo, which are concluded from the experiment observations. In this part, we will especially show the limitations of Open-Flamingo that will damage the ICL performance of VQA. Then in Section~\ref{sec 4.2}, we will show which configuration strategies can be used to alleviate these limitations for improving the performance.

%能从task recognition和task learning的角度去写这个文章吗？一切都往这个主题上靠？现在可以看出vqav2数据集上很多策略都不显著，而在另外两个数据集上相对显著。这是vqav2这个数据集的原因吗？是vqav2的图片或者回答比较正常，其他的数据集图片或者回答不正常，所以额外的找相似的图片有很大的帮助？其他数据集如果因为图片/回答不正常，那么找到相似的图片/回答是一种帮助task recognition还是一种帮助task learning呢？
%发现3个数据集的特点不一样，那么虽然都是vqa，但其实可能没有过于通用的strategy，这个时候就需要去分析3个数据集的特点了，所以dataset这一节很重要。

%直觉上，random sampling的话更多体现在task recognition上，而找相似的image/question是为了帮助task learning，这个能从论文里找到依据吗？如果是这样，那么在vqav2情况下，siir相比rs提升不大，说明task recognition在起作用，但是为什么sqqr比rs差呢？是找相似的question形成了干扰吗？

%现在的几个结论：
%1.对于不同数据集而言，找相似的图片依然是最管用的，但是不同的数据集以及不同的of版本上提升不同。
%2.可以观察到task recognition的作用大于task learning，或者说更显著吧，比如在mismatch时影响不大。还有一些其他实验，这个可能也看数据集。
%3.language model能力强，那么instruction有效，尤其是shot数少的时候，比如0 4 shot，是不是可以认为instruction也让model获得了一定的task recognition能力

%v1上面大多数当shot数增加，效果还是在变好，但是不明显，这个怎么解释？
%在v1中，大多数策略都是在shot数少的时候提升大，shot数大的时候提升小，比如4-shot时，rs为44，siir 47，siir_0 50,SQAQAR(SIIR--) 52,这个怎么解释？
%在v2中，很多v1中有效的策略到v2都无效了，这是为什么？比如v1中siir，sqqr和rs相比都有提示，尤其是4-shot的时候，但是在v2中，sqqr，diir相比rs下降了，这是为啥？

%在v1中，SQAQAR（replace Q）是50，SQAQAR（replace I）是65，说明当ICE中question-answer和query的question-answer pair匹配时而image不匹配时，vqa结果好，说明这个时候language的影响力是要大于vision部分的。
%以上观察是不是说明bias可能来自LLM，即不给image的时候可能qa效果也不错，所以也可以把所有的image去掉，只测qa，看看有没有什么影响。

%SQAQAR（sole），即ice里只有一个qa对是和query一样的，剩下的是random sample，有54，那么是不是说明在ICE里，只要找到一个正确的question-answer pair就可以提升性能了呢？是不是暗示我们可以考虑这样一个方法：1.先想办法给query生成一个或者多个pseudo answer，然后再用这些pseudo answer去retrieve一些ICE看看性能。2.那么怎么生成多个pseudo answer呢？付嘉乐的那种想法可以吗？就是把最后的softmax给relax下，用一个template控制下？
%但是这种方法不一定有用，因为SQAQAR（sole）其他的example是随机采样的，所以可能这些example不会产生干扰，但是如果用pseudo answer来retrieve的话，对于retrieve到的examples，可能会形成干扰

%mismatch的情况有影响，但是都不大，结合前面的结论可能真的是vqa-icl里面task recognition的作用比task learning的要大

%siir sqqr在vizwiz上有效果，shot少的时候siir好非常多，然后shot数多了之后siir和sqqr的差距不明显，甚至和rs的差距不明显，可以认为是这么多shot里task recognition做的更好，这里的task recognition指的是在vizwiz这个数据集上更适配了，而task learning做的不够好，或者说task learning提升不是很大，这说明现在的open-flamingo的task learning能力还不够。

%flamingov2用instruction效果有点提升，而v1不行，说明v2的language module比较好，然后用instruction之后在shot数少的时候好，而且instruction的意义就在于task recognition，所以还是说明了现在的vlm对task recognition比较有用。

%siqr和sqir为什么在shot数多的时候差3个点？用image找question，可能找到一些视觉信息都在的question，用question找image，可能question中就没有什么视觉信息，所以找的图片不够好，然后shot数多了之后可能找的图片更不好了，但是用了qa之后(这个有点奇怪，为啥用image去找文本 带answer的效果差，用文本去找image 带answer的效果好)

%为什么vizwiz数据集上sqaqar比sqaqar(siir)差，用了伪答案效果比用真实答案好？这个理由是不是因为这个：由于vizwiz数据集gt answer太长，很少有重复的，所以带answer搜索也搜索不到非常接近的qa pair，就算有copy effect，但是因为找不到相似的qa pair，抄都不好抄，然后ofv2生成的answer pattern简单点，反而有助于去找到一些不错的qa pair，比如说answer pattern简单，就能找到不错的qa pair，然后让效果变好？

%强相似是最好的，即image相似，question相似（SIIR_2），这个在v1，v2上以及多个数据集上都有观察到，比如v2上面大多数策略在32shot时都会降低，但是用siir_2会一直提升，说明强相似找的example更有用。

%v1 v2的区别，不同策略的倾向性，不同策略在不同数据集上的效果

%ofv2的实验里，vqav2的sqqr比rs差 是因为找相似question引起了干扰吗？这个可以细化到每个问题类型看看结果。在v1情况下，sqqr效果好，而v2下，sqqr效果不行，可能是因为v2的llm很强，所以language带来的干扰变大？
%v1里sqqr的提升比siir大，但是v2里，sqqr提升比siir小。

\begin{figure*}[htb]
  \centering
  \includegraphics[width=17cm]{figure/visualized2.pdf}
  \caption{visualizations.}
  \label{fig:visualized}
  % \vspace{-0.2in}
\end{figure*}


\subsubsection{The Characteristics of Open-Flamingo}

% !!!: 首先需要一张gold＞mismatch＞visual tr＞linguistic tr的图

\noindent\textbf{Task Recognition (TR) Plays More Significant Roles than Task Learning (TL).}
% ~\cite{What In-Context Learning “Learns” In-Context:
% Disentangling Task Recognition and Task Learning} disentangles ICL into two components: Task Recognition (TR) and Task Learning (TL). TR involves recognizing the task based on the demonstrations, \eg, the data distribution of the task, and applying pre-trained priors of LLM. TL, on the other hand, focuses on learning the correct input-output mapping from the demonstrations, which can be seen as comparable to few-shot learning without fine-tuning.
% Building upon this, we further hypothesize that TR, particularly in the context of ICEs, helps the model identify the potential answer space within all tokens. Specifically, for visual TR, it involves extracting information from the image to determine the label space, which could consist of various tags or tag phrases related to the image. On the other hand, for linguistic TR, it focuses on recognizing aspects of the question and answer, including the format, input distribution, and answer space. For example, it recognizes the form of the answer (single word or a few-word phrase instead of a complete sentence) and potential answers based on the question (\eg, a question asking for color will have a limited set of color options as potential answers).
% TL, on the other hand, refers to the model learning the mapping between the inputs (image and question) and outputs (answer) presented in the ICEs. It utilizes the query image and question to find the correct answer within the intersection of the answer spaces obtained from visual and linguistic TR.
% 如图x（tr，tl示意图）
% ~\cite{What In-Context Learning “Learns” In-Context: Disentangling Task Recognition and Task Learning} observed that mismatches have minimal impact on ICL. ~\cite{xxx} mentioned that as long as three conditions are satisfied (format, input distribution, and label space), ICL in Language Models (LLMs) can perform well. This suggests that TR plays a more significant role than TL in LLMs. 
As discussed in Section~\ref{xxx}, the ICL ability of a LVLM can be decoupled into two aspects, which are TR and TL.
The first conclusion about the characteristics of Open-Flamingo is that \textit{TR plays more significant roles than TL}, which can be supported by two experiment observations.

Firstly, as stated in ~\cite{tr&tl},  the performance of in-context TR is expected to show no significant improvement when using more demonstration shots since xxxx. Conversely, as the shot number of the demonstration increases, the TL aspect of the model should exhibit better performance since xxx.
From \cref{fig:icl_result}, we observe that when shot number increases, the accuracy does not consistently increase. For example, when retrieving image from image via similarity (I-I-S) in VQAV2, increasing the shot number from 8 to 16 yields a smaller accuracy gain (1.15 points) than from 4 to 8 (2.59 points), and notably, accuracy declines when the shot number rises from 16 to 32. Similar observations can be found when using other strategies in both VQAv2 and OKVQA. Thus, it is safe to conclude that TL performs worse than TR in the ICL ability of Open-Flamingo.

%对于vizwiz数据集，因为其image是盲人拍的，所以图片质量不行，且文本质量也不行，所以image and text distribution和训练数据不是很match，这种情况下，ICE多了，VLM可以更好的识别vizwiz的data distribution，也就是task recognition做的越好，但是不能说明task learning做的好。
% For the results in VizWiz, we observe that the accuracy increases largely when 
% Although the accuracy consistently increases when shot number increases in VizWiz, the major reason is that the image and text quality of this dataset is lower than the commonly used image-text pair and using more ICEs will help Open-Flamingo recognize the data distribution
Secondly, Table~\ref{xxx} shows the results where the disturbed demonstrations are used, we can observe that, anti-intuitively, when the disturbed triplet demonstrations are used, the VQA performance does not significantly degrade. For example, when we disturb all the input-output mappings, the accuracy of xxx on xxx dataset only degrades xxx. Such phenomenon can be explained from the perspectives of TR and TL. Specifically, TR focus on recognizing the question format, input distribution, and label space from the demonstrations, which can be provided from the disturbed demonstrations as the non-disturbed ones. TL needs to capture the correct input-out mapping while the disturbed demonstrations can not provide such knowledge. In this way, it can be concluded that TR is less affected by the the disturbed demonstrations than TL. Then since we observe that the ICL performance is not heavily affected when the demonstrations are disturbed, we can conclude that TR plays more pivotal role than TL here. 

Besides these two experiment observations support the claim, we follow~\cite{tr&tl} to design an experiment to further validate it. Specifically, we xxxxx. Table xxx shows the results, we can find that xxxx. Such observation further confirm our claim.

% we also create mismatched input-output mappings to check whether this heavily degrades the accuracy, where the results are reported in Figure~\ref{fig:xxx} and two kinds of mismatching are considered: xxx denotes the question-answer pair is not related to the image and xxx denotes the answer is not correctly answered to the given question. 
% Based on the results of our mismatched triplet experiment, we observe a similar phenomenon in LVLM. When the input-output mappings are disrupted, the performance does not significantly degrade. For example, when we disturb all the input-output mappings, the accuracy of xxx on xxx dataset only degrades xxx. 
%第一个xxx是策略，比如rs还是siir，第二个xxx是dataset名称，第三个xxx是降低了多少个point。
% Such observation suggests that mismatched mappings do not heavily affect the accuracy, which validates that TR plays more significant roles than TL in LVLM since the major function of TR is to recognize the data distribution instead of learning the correct mapping as illustrated in \cref{fig:more_trtl}.

% Thirdly, to further confirm this claim, we follow~\cite{What In-Context Learning “Learns” In-Context:
% Disentangling Task Recognition and Task Learning} to carry the following additional experiments. 


% \noindent\textbf{More In-Context Examples lead to Worse Performance.}
% %1.先写conclusion，然后写哪些实验可以观察到，为了进一步验证，我们又补充了一些实验


\noindent\textbf{Copying effect interferes with model inference.}
% （引copying effect）发现lm进行single sentence classification时，会无视正误，直接在ice中copy相似文本的label。在我们的实验中，发现vlm同样存在copying effect。
% 上一节提到的，ice对tl产生干扰的一种极端情况就是copying effect，这时model几乎没有经过任何的推理（short cut）就直接将问题指向了ice里见过的答案，如图xx（trtl示意图）所画。
Prior research in the field of NLP has confirmed that using similar questions as in-context examples can enhance performance. However, our experiments revealed an anti-intuitive situation:
%这边要写下不是所有的similarity based methods可以提升性能，比如Q-Q-SE就没有，而且这边要说一下是language encoder有点强导致的
Q-Q-SE does not consistently result in performance improvement. On the contrary, sometimes it even leads to a decline in model performance.
As shown in \cref{fig:icl_result}, its performance on VQAv2 was inferior to RS. However, its counterpart experiment QA-QA-S showed stable and significant improvements in the model's performance.

~\cite{lyu2022copyingeffect} have discerned a tendency for LMs to directly replicate labels from ICEs that exhibit textual similarity, showcasing the \emph{copying effect}. 
% Essentially, rather than truly understanding or classifying the input, the model often opts for a shortcut, extracting and reproducing labels from similar texts within its ICEs, thereby showcasing the \emph{copying effect}. 
Additionally, when exploring the demonstration configuration for image captioning,  ~\cite{wylnips} has also discovered that when the query image is similar to the demonstration, a shortcut inference occurs, utilizing the in-context caption to generate the caption.
In our experiments, a parallel behavior was identified, suggesting that this effect isn't limited to text-only models but also extends to models that process both visual and textual data and this phenomenon appears to be generalizable across LVLM tasks.

% During the Q-Q-S experiment, we noticed that it did not consistently improve the model's performance. As shown in Table X, its performance on VQAv2 was inferior to RS. However, its counterpart experiment QA-QA-S showed stable and significant improvements in the model's performance. 
Upon analyzing the model's output, we discovered that the model exhibites answer copying behavior from the demonstration. 
Specifically, as illustrated in \cref{fig:visualized}, when the demonstration included a question highly similar to the query, the model tended to directly copy the answer from the demonstration, taking a "shortcut" rather than comprehensively processing the input to derive an answer. 
We speculate that this could be due to the limited TL capability of Open-Flamingo. As a result, it is influenced by the bias in the input-output mapping of the demonstration, leading to erroneous learning of the mapping relationships and resulting in overfitting.
In \cref{fig:visualized}, when inquired about the pattern of bed sheets (the correct answer being 'zebra'), Q-Q-SE veered off, opting for 'alligator and bear'—answers previously observed in ICEs, even though they bore no relation to the image in question. 
In \cref{table:copying rate}, we compute the probability of the model's predicted answer appearing in the demonstration and discover that the Q-Q-SE approach has a 70\% probability of a copying effect, while the QA-QA-S approach has an 80\% probability. Even when there is only one example in the demonstration that is similar to the query (\cref{table:sole copy rate}), the probability of copying the sole answer can still reach 47\%. Furthermore, even after replacing the answer of this in-context example with an incorrect one, there is still a 37\% chance that the model will directly copy this erroneous answer without engaging in any reasoning.

\begin{table}
  \centering
  \scalebox{0.85}{
  \begin{tabular}{l c c }
    \toprule
       & ofv1 & ofv2\\
    \midrule
    Q-Q-SE & $77.26$ & $79.84$ \\
    QA-QA-S & $87.74$ & $89.47$ \\ 
    \bottomrule
  \end{tabular}
  }
  \caption{The copying rate analysis using 16-shot results. }
  \label{table:copying rate}
  % \vspace{-0.1 in}
\end{table}
% use 16 shot

\begin{table}
  \centering
  \scalebox{0.85}{
  \begin{tabular}{l c c}
    \toprule
       & ofv1 & ofv2\\
    \midrule
    Total & $42.23$ & $ $ \\
    \quad correct & $47.39$ & $ $ \\
    \quad incorrect & $37.07$ & $ $ \\ 
    \bottomrule
  \end{tabular}
  }
  \caption{The copying rate of demonstrations with a single similar question and randomly selected remaining questions(16-shot).}
  \label{table:sole copy rate}
  \vspace{-0.2 in}
\end{table}

\noindent\textbf{Texts is more essential than images.}
% 1、mismatch系列实验中，sqqr更换image下降1个点，更换answer下降5个点；
% SQAQAR（replace Q）下降15个点，SQAQAR（replace I）几乎没有明显下降；
% 这些现象解释为在目前做icl的VLM中，语言端的影响远远大于视觉端，然而更具体地应解释为：
% ice的文本给模型带来的引导比ice的图像更大。
% 可以认为model在进行tl的时候，会被ice的样本所影响，这种影响可能是正向的，可以帮助model更准确地指向正确答案（比如目前认为siir是这样的影响，okvqa上得sqqr也是如此）；同时这种影响也可能是干扰，导致找到的answer偏移到了别的answer space里（这也许是sqqr在vqav2上有时候表现反而不好的原因，具体会在similarity-based一节详细讨论）
% 2、instruction
% 此外，对于language model能力更强的ofv2其被文本影响更大，除了更容易被干扰以外（3.3节），在v2上instruction策略有效，尤其是shot数少的时候，帮助模型进行tr，从更少的ice中学到任务信息。
In the study of ICL using Open-Flamingo, a salient observation emerges: \textit{texts play a considerably more pivotal role than images.} This observation is supported by two experimental phenomena.

Firstly, we observe that Open Flamingo exhibits a heightened sensitivity to text quality. When the quality of the textual input is compromised, the model exhibits a more pronounced decline in performance. In the Q-Q-S experiment, replacing the image led to a minor 1-point decrease in performance, while replacing the answer resulted in a significant 5-point drop. In the QA-QA-S experiment, substituting the question (replace Q) led to a notable decline of 15 points, whereas replacing the image (replace I) did not cause a significant decrease.
Secondly, from Figure X, it is evident that replacing the text with noisy text leads to a more significant performance decline compared to replacing the image with a blurred image. This finding highlights the heightened importance of text in LVLM ICL, emphasizing that linguistic TR plays a more substantial role than visual TR.
We hypothesize that this phenomenon occurs because that for Open-Flaming, the language module is more powerful than the visual module. 


% These phenomena can be interpreted as an indication of the prevailing influence of language over vision in the current VLMs when utilizing ICL. More specifically, the guiding influence or hint provided to the model by the in-context example text (ICE-text) appears to be more potent than that provided by the in-context example image (ICE-image). It can be inferred that when the model engages in task learning, it can be influenced by the ICE samples. This influence can be advantageous, guiding the model more accurately towards the correct answer, as evidenced by SIIR and the OKVQA dataset with SQQR. Yet, it can also serve as a distractor, diverting the response to a different answer space. This might elucidate why SQQR sometimes underperforms on the VQAv2, which will be elaborated upon in Section xxx.

% The results derived from the more linguistically advanced model, Open-Flamingo v2, further underline the critical role of text in ICL. This model, owing to its heightened language prowess, is even more susceptible to textual influences. The strategy to use instructions proves effective, especially when the number of shots or ICEs is limited. This indicates that the instruction aiding the model in task recognition, enabling it to glean task-specific information from a limited set of ICEs.

\noindent\textbf{Not All Effective NLP Strategies Apply to LVLM.}
% pjw：从tr tl角度看，一些策略例如交换顺序和陈述句这种nlp的方法无效，是因为其没有太大影响到tr tl能力，甚至影响了ice结构后会影响tr能力
% yx：我感觉这一段要不要放这边也是个问题，如果放这，就应该先写，虽然前面发现text比image作用大，这个是因为VLM中的language model部分强于visual部分，但是也不是任何的NLP中有用的ICL策略都在VLM中起作用。然后先说变成declarative的这个为什么差，有什么理由吗？先写变成declarative因为这个和language encoder直接相关，顺序那个好像和language encoder不直接相关。这一段的写作还要想想，现在这种写法不合适。
However, it is worth noting that some strategies which exhibit promising results in NLP tasks, may not necessarily have the same effectiveness for LVLM. Strategies such as changing the orders of demonstrations or changing question-answer pairs into declarative sentences struggled to achieve substantial improvements in VQA task. We consider that these strategies do not improve the task recognition or task learning capabilities during ICL. Given the limited number of demonstrations, the impact of their order in visual-language models is considerably less pronounced than the influence of long text sequences on language models. And adding the declarative sentences into demonstrations might perturb the format of the demonstrations, potentially impeding the task recognition capability of the model.
% ↑可以写成改成declaration之后，input distribution和预训练很不一样，导致tr做不好了

\begin{table*}
  \centering
  \scalebox{1}{
  \begin{tabular}{@{}l | c c | c c | c c@{}}
    \toprule
       & OFv1-VQAv2 & OFv2-VQAv2 & OFv1-VizWiz &  OFv2-VizWiz & OFv1-OKVQA & OFv2-OKVQA \\
    \midrule
    Baseline(RS)       
    & $45.97$ & $49.94$ & $27.00$ & $27.21$ & $36.13$ &$36.68$\\
    RS-mismatch(I)     
    & $45.13$ & $49.73$ & $00.00$ & $35.12$ & $00.00$ &$36.16$ \\
    RS-mismatch(A)     
    & $45.65$ & $48.94$ & $00.00$ & $15.03$ & $35.56$ &$29.88$ \\
    I-I-S              
    & $48.48$ & $51.66$ & $38.21$ & $39.10$ & $39.87$ &$38.35$ \\
    I-I-S-mismatch(QA) 
    & $47.76$ & $49.94$ & $00.00$ & $26.73$ & $37.78$ &$35.82$ \\
    I-I-S-mismatch(A)  
    & $47.64$ & $50.40$ & $00.00$ & $11.48$ & $34.92$ &$29.55$ \\
    Q-Q-S 
    & $49.53$ & $48.83$ & $30.69$ & $34.17$ & $40.31$ &$37.52$ \\
    Q-Q-S-mismatch(I)  
    & $48.01$ & $46.21$ & $00.00$ & $31.95$ & $38.79$ &$33.25$ \\
    Q-Q-S-mismatch(QA) 
    & $45.32$ & $48.98$ & $00.00$ & $26.45$ & $37.39$ &$35.52$ \\
    Q-Q-S-mismatch(A)  
    & $47.18$ & $42.72$ & $00.00$ & $15.42$ & $29.47$ &$20.50$ \\
    \bottomrule
  \end{tabular}
  }
  \caption{The results of mismatching the triplet with average values for 4-shot and 8-shot.}
  \label{table:result}
\end{table*}

\begin{table}
  \centering
  \scalebox{0.5}{
  \begin{tabular}{@{}l|c c| c c| c c|@{}}
    \toprule
       & ofv1-vqav2 & ofv2-vqav2 & ofv1-vizwiz &  ofv2-vizwiz & ofv1-okvqa & ofv2-okvqa \\
    \midrule
    QA-QA-S       
    & $65.705$ & $61.495$ & $41.455$ & $41.455$ & $52.49$ & $47.845$ \\
    QA-QA-S(repace I)    
    & $65.52$ & $ $ & $41.09$ & $40.66$ & $51.31$ & $46.88$ \\
    QA-QA-S(repace Q)             
    & $50.62$ & $60.615$ & $40.31$ & $40.16$ & $40.245$ & $33.04$ \\
    \bottomrule
  \end{tabular}
  }
  \caption{The results of replacing questions and images of QA-QA-S with average values for 4-shot and 8-shot.}
  \label{table:replaceQ&I}
\end{table}


% copying effect的数据统计，包括copy rate etc
% captioning也有short cut inference

% Our earlier discussions highlight how ICEs can at times interfere with task learning (TL), skewing the model's output. The copying effect can be seen as an extreme embodiment of this interference. Instead of performing genuine reasoning based on both visual and textual cues, the model, under the influence of the copying effect, gravitates towards directly linking the query to an answer it has previously seen within its ICEs. From figure xxx, when copying effect happens, the model takes a "shortcut" rather than comprehensively processing the input to derive an answer.

% % fine-grained结果：vqav2不同类型的copy rate不一样；label space越简单，copy effect越明显

% of两个版本的比较
\noindent\textbf{Open Flamingo V1 vs V2: Differences in LVLM Models.}
% v2是用了更强大的语言模型，也预训练了更多的数据，因此有了更好的表现（rs baseline）（tr更强了？
% tl能力更强（比如mismatch实验中效果下降更多）
% v2的qaqas不如v1是因为copying effect更严重（语言模型更强大?）
% instruction有效（语言模型更强大）


\subsubsection{Effective Demonstration Configuration Strategies}
In the previous section, we conducted experiments to observe the characteristics of a current state-of-the-art LVLM for ICL. While it is considered a strong model, we identified some limitations, such as weak TL capabilities, a comparatively weaker visual encoder compared to the language decoder, and the presence of copying effect. Now, the question arises: How can we strategically enhance the capabilities of this limited LVLM for VQA ICL purposes?

% \noindent\textbf{ensemble.}

\noindent\textbf{Similar images and texts lead to better performance.}
% nlp的xxx论文证明在nlp icl里面similarity是有效的，在我们的实验里，首先整体上看，similarity-based方法是有效的，不过具体情况因数据集和模型而异。
% 1、siir普适成功
% 认为siir是补充信息的作用，讨论表格数据+给个例子（蔬菜汤）
% 2、sqqr的干扰
% 过于相似的文本会对model的tl产生干扰，给例子（鳄鱼小熊）
% 3、强相似是最好的，即image相似，question相似
% 更进一步，在similarity的基础上，对ices进行重排序的强相似方法能进一步提高模型的表现，在两个模型和三个数据集上都可以看到+的方法比base方法有进一步的提升，这证明在model不受内容过于相似的文本干扰时，对于vlm来说无论是visual还是text的similar ice都可以帮助模型的tr和tl
~\cite{xxx} demonstrates that similarity-based methods are effective in NLP in-context learning. From our experiments, it is generally observed that similarity-based methods are also effective in LVLMs although the specific results may vary depending on the dataset and model used.

Firstly, I-I-S demonstrates consistent success across varied models and datasets. When images are similar, LVLMs improve VQA reasoning for the query by learning the mapping relationships within the demonstration. This compensates for any information that may have been missed or incorrectly recognized during the visual TR stage.
% Even if the model misinterprets certain visual elements of the query image, the prior knowledge from demonstration can rectify or supplement the missing or misunderstood information. 
For instance, in \cref{fig:visualized}, while both RS and Q-Q-S could only recognize the term 'vegetable' for an image of a soup can, I-I-S, using ICE-images, identified it as a 'Progresso vegetable soup'.
Quantitatively, as illustrated in Table XXX, I-I-S consistently boosts LVLM performance. On the VQAv2 dataset, an average increment of 2 points is observed; on OKVQA, a rise of 3-5 points; and the most prominent uplift, a remarkable 10 points, is seen on VizWiz. We postulate that the less-than-ideal image quality in VizWiz makes the retrieval of similar images invaluable, aiding Open-Flamingo in pinpointing a more accurate label space.

% Secondly, despite the above success, our experiments also spotlighted cases where high textual similarity could deter model performance. Particularly on the Open Flamingo V2(with an advanced language model than V1), Q-Q-S at times underperformed compared to random selection. This could be attributed to the model being overly influenced by the demonstrations present in the ICEs, deviating from its natural reasoning abilities. For instance, in one VQAv2 example in figure xx, when inquired about the pattern of bed sheets (the correct answer being 'zebra'), Q-Q-S veered off, opting for 'alligator and bear'—answers previously observed in ICEs, even though they bore no relation to the image in question. Such outcomes highlight the model's susceptibility to ICE influence, even manifesting the aforementioned 'copying effect.' 
% Notably, in certain circumstance, the model correctly answered under RS but was misdirected by Q-Q-S to replicate ICE answers. The discord between image visual cues and the model's answer was blatant, further accentuating Q-Q-S's unexpected shortfalls. Such discrepancies perhaps point towards the model's limited task learning capacity, causing it to be unduly influenced by biases in ICEs, resulting in overfitting. The variations between the performances of the two versions of Open Flamingo could be attributed to V1 having a less potent language model than V2, making it less prone to textual influences.
Secondly, the Q-Q-S approach also brings improvements, although these enhancements are not consistently stable due to the presence of the copying effect. However, as shown in Table X, for the VizWiz dataset with lower-quality text and the OKVQA dataset requiring additional knowledge, demonstrations containing similar questions and reference answers still assist the model in finding the correct answers.

% Thirdly, in approach section, we introduced a unique similarity-based retrieval methodology named "Strong Similarity". This method builds upon the foundation of retrieving similar images or questions. Specifically, it reorders samples that are visually analogous to the query based on the similarity of their associated questions. Alternatively, when commencing from a premise of similar questions, it repositions them according to the likeness of their associated images. 
Thirdly, in the approach section, we introduced a unique retrieval method that reorders the retrieved in-context examples based on their similarity in another modality. This method retrieves similar images or questions and rearranges them based on the similarity of their associated questions or images.
As \cref{fig:icl_result} shows, When applied to two distinct models and across three varied datasets, this method consistently showcased superiority over base methods. Such findings suggest that, both visually and textually similar in-context examples can greatly enhance the performance of LVLMs in TL. In multimodal tasks, demonstrations that exhibit similarity in both modalities have the maximum potential to improve LVLM performance.
% pjw：我们instruct的实验其实也不是很多，主要就是观察到在v2上效果优于v1，以及0shot上提升明显，另外在okvqa上试了各种instruction，都有一些提升，主要想继续从tl这个角度解释

% \begin{table*}
%   \centering
%   \scalebox{0.82}{
%   \begin{tabular}{@{}l c c c c p{12cm}@{}}
%     \toprule
%     Setting   & 0 shot & 4 shot & 8 shot &   16 shot & instruction \\
%     \midrule
%     Baseline(ofv1-vqav2) & $43.29$ & $44.56$ & $47.38$ & $48.71$ &  \\
           
%     Instruct(ofv1-vqav2) & $42.88$ & $43.75$ & $46.91$ & $48.67$ & According to the previous question and answer pair, answer the final question. \\
%     \midrule
%     Baseline(ofv2-vqav2) & $47.39$ & $48.82$ & $51.05$ & $50.89$ &  \\

%     Instruct(ofv2-vqav2) & $50.90$ & $49.93$ & $52.71$ & $50.95$ & According to the previous question and answer pair, answer the final question. \\
%     \midrule
%     Baseline(ofv2-vizwiz) &  & $22.07$ & $32.35$ & $39.01$ &  \\

%     Instruct(ofv2-vizwiz) &  & $25.7$ & $34.71$ & $39.32$ & According to the previous question and answer pair, answer the final question. \\
%     \midrule
%     Baseline(ofv2-okvqa) & $34.56$ & $33.8$ & $38.01$ & $39.92$ &  \\

%     Instruct(ofv2-okvqa) & $38.06$ & $35.72$ & $39.38$ & $40.46$ & According to the previous question and answer pair, answer the final question. \\

%     Instruct(ofv2-okvqa) & $40.23$ & $36.45$ & $40.17$ & $41.11$ & Consider the semantic relationship between the question and the image. \\

%     Instruct(ofv2-okvqa) & $39.4$ & $35.53$ & $40.19$ & $40.02$ & You will be engaged in a two-phase task. Phase 1: Absorb the information from a series of image-text pairs. Phase 2: Use that context, combined with an upcoming image and your own database of knowledge, to accurately answer a subsequent question. \\
%     \bottomrule
%   \end{tabular}
%   }
%   \caption{The results of using instructions.}
%   \label{table:instruction}
% \end{table*}

\begin{table}
  \centering
  \scalebox{0.85}{
  \begin{tabular}{@{}l l l c c c c@{}}
    \toprule
    Method & Model & Dataset & 0 shot & 4 shot & 8 shot &   16 shot \\
    \midrule
    RS & OFv1 & VQAv2 & $43.29$ & $44.56$ & $47.38$ & $48.71$  \\
           
    Instruct1 & OFv1 & VQAv2 & $42.88$ & $43.75$ & $46.91$ & $48.67$ \\

    RS & OFv2 & VQAv2 & $47.39$ & $48.82$ & $51.05$ & $50.89$  \\

    Instruct1 & OFv2 & VQAv2 & $50.90$ & $49.93$ & $52.71$ & $50.95$ \\

    RS & OFv2 & VizWiz  &  & $22.07$ & $32.35$ & $39.01$   \\

    Instruct1 & OFv2 & VizWiz &  & $25.7$ & $34.71$ & $39.32$ \\

    RS & OFv2 & OKVQA & $34.56$ & $33.8$ & $38.01$ & $39.92$  \\

    Instruct1 & OFv2 & OKVQA & $38.06$ & $35.72$ & $39.38$ & $40.46$  \\

    Instruct2 & OFv2 & OKVQA & $40.23$ & $36.45$ & $40.17$ & $41.11$  \\

    Instruct3 & OFv2 & OKVQA & $39.4$ & $35.53$ & $40.19$ & $40.02$ \\
    \bottomrule
  \end{tabular}
  }
  \caption{The results of adding instruction at the beginning of the in-context sequence. The instruction of Instruct1: ``According to the previous question and answer pair, answer the final question.". The instruction of Instruct2: ``Consider the semantic relationship between the question and the image." The instruction of Instruct3: ``You will be engaged in a two-phase task. Phase 1: Absorb the information from a series of image-text pairs. Phase 2: Use that context, combined with an upcoming image and your own database of knowledge, to accurately answer a subsequent question."}
  \label{table:instruction}
\end{table}

\noindent\textbf{Instructions can enhance the performance of linguistically advanced model.}
In scenarios with limited demonstrations, the directive information of the instruction offsets the diminished TL capability of the model, resulting in a pronounced enhancement. As evident in \cref{table:instruction}, the Open-flamingo v2 model has shown pronounced improvements across various datasets by adding instruction before the demonstrations. This is especially evident in settings with fewer shots, for instance, adding instructions to the 0-shot experiment on the OKVQA dataset leds to a 3.5 points increment. Additionally, models with weak TL capability may struggle to improve by using instructions, as \cref{table:instruction} shows, the effect of instruction is negligible in the v1 model. Considering the complexity of the VQA task in the OKVQA dataset, we devised diverse instructions to observe the results in the OKVQA dataset. Our findings indicate that both succinct, clear instructions and detailed, hierarchical ones can improve the TL capability of the model better.
% The strategy to use instructions proves effective, as evident in Table xxxx, the Open-flamingo v2 model has shown pronounced improvements across various datasets by adding instruction before the demonstrations. This is especially evident in settings with fewer shots, for instance, adding instructions to the 0-shot experiment on the OKVQA dataset leds to a 3.5 points increment. In scenarios with limited demonstrations, the directive information of the instruction offsets the diminished TL capability of the model, resulting in a pronounced enhancement. However, it is worth noting that this enhancement is more effective in linguistically advanced models, as Table xxx shows, the effect of instruction is negligible in the v1 model. Considering the complexity of the VQA task in the OKVQA dataset, we devised diverse instructions to observe the results in the OKVQA dataset. Our findings indicate that both succinct, clear instructions and detailed, hierarchical ones can improve the TL capability of the model.
 %The results derived from the more linguistically advanced model, Open-Flamingo v2, further underline the critical role of text in ICL. This model, owing to its heightened language prowess, is even more susceptible to textual influences. 


\noindent\textbf{Pseudo answers have potential for expeditious enhancement of performance.}
%看看有没有那种受启发然后刷分的方法，比如生成伪造的answer再去检索。
% 所有数据集和模型上，伪答案都有一定的提升
% specially，某些数据集上甚至  使用伪答案比gt好
Inspired by the advantage of the shortcut in QA-QA-S, we have designed the A-PA-S method. Since ground truth is unavailable in practical applications, we adopt a multi-round reasoning approach. We utilize the initially generated pseudo-answers with lower accuracy in the first round as the input for QA-QA-S retrieval, using the retrieved results as the demonstration for the second round.
From the results in \cref{table:Pseudo answers}, it can be observed that the second round of A-PA-S generally improves upon the results of the first round. This demonstrates the effectiveness of utilizing pseudo-answers with the copying effect as a viable strategy for improving accuracy.

\begin{table}
  \centering
  \scalebox{1}{
  \begin{tabular}{@{}l  c  c  c @{}}
    \toprule
       & vqav2 & vizwiz & okvqa \\
    \midrule
    RS 
    & $48.82$ & $22.07$ & $33.80$ \\
    A-PA-S(RS)    
    & $49.85$ & $30.02$ & $38.92$ \\
    I-I-S              
    & $50.02$ & $36.30$ & $36.46$ \\
    A-PA-S(I-I-S)
    & $50.57$ & $38.37$ & $39.34$ \\
    \bottomrule
  \end{tabular}
  }
  \caption{The performances of A-PA-S(4-shot).}
  \label{table:Pseudo answers}
\end{table}

==> sec/intro_temp.tex <==
\section{Introduction}
\label{sec:intro}
% The rise of Large Language Models (LLMs) has profoundly impacted the field of machine learning. With the expansion in model size and training data, their capabilities have seen a marked increase. This evolution has paved the way for innovations such as prompt engineering and in-context learning. These developments have streamlined approaches to various tasks, obviating the need for task-specific training. In the realm of in-context learning, it has been observed that the configuration of in-context examples plays a pivotal role in determining performance. This realization has led to intensified research efforts aimed at refining these configurations to optimize results. While prompt engineering was an initial focus, the emphasis has progressively shifted to the more adaptable in-context learning.


% With the triumph of LLMs and the advent of in-context learning capabilities, researchers in the vision-language domain have been inspired to design large models that harness the power of in-context learning. Early endeavors in this direction include models like 'Frozen' and the subsequent 'Flamingo', both of which introduced large vision-language models capable of in-context learning.

% However, a gap exists in the vision-language domain. While there has been some exploration into the impact of different in-context configurations on performance, especially in image captioning, there's a noticeable dearth of research in another veteran task of the vision-language domain: Visual Question Answering (VQA). Our study primarily seeks to bridge this gap by investigating how various VQA configurations influence performance.

% VQA presents a more intricate scenario compared to image captioning. While in-context examples for image captioning typically comprise a binary tuple of image-caption, VQA involves a triad: image, question, and answer. This complexity necessitates a more comprehensive consideration of factors. To exhaustively explore the influence of diverse in-context configurations on performance, we've devised numerous configuration strategies. These include seeking images or texts (question-answer pairs) similar to the query example. Drawing inspiration from NLP, we've adapted many strategies used in question-answer in-context learning to the vision-language domain. Examples include mismatching elements within the image-question-answer triad or altering the sequence of in-context examples. Furthermore, given that model scale has been observed to influence in-context configurations in the NLP domain, we employed two scales of large vision-language models to assess the impact of scale on outcomes. In doing so, our strategies also offer insights into the nuances between different model scales, potentially demystifying the "black box" of large models and aiding researchers in better understanding these behemoths.

%v1
%由于真实世界过于复杂，很难直接从内部去理解它，所以科学家会使用由外向内的方式来理解世界，比如把这个世界作为一个black box，然后做控制变量的实验去观察改变一些input，会得到什么样的output，然后根据这种input-output的反馈来做些猜想，之后再做更多的实验去验证自己的猜想。对于AI领域，虽然现在流行的foundation model没有真实世界那样复杂，但是也很难从内部直接去搞懂他，所以研究者使用了一些控制变量的方法从外部输入一些数据进去看看返回的是什么，通过由外向内的方式研究大模型。

%其中比较典型的方法是使用prompt engineering的方式去观测LLM，比如改变prompt sentence作为input，看看对解决一个任务有什么影响，然后推测一些LLM的性质。在prompt engineering中，ICL也是一种特殊的prompt engineering，只要把不同的ICE串起来，就可以看成是一个特殊的prompt。由于可以用多种方式来configure ICE,所以通过控制ICL来观察LLM，从而推测其功能也是一种很好的方法，比如有研究者发现可以把大模型的ICL能力disentangle为Task recognition和Task Learning，也有的研究者发现LLM有copy effect。

%最近，看到LLM的成功，vision-language领域的研究者也开发了有ICL能力的大模型，flamingo和对应的开源版本open-flamingo。但是类似于以上的研究还不多。为了弥补这个差距，在这个study中，我们选用VQA为case study去研究现有的VLM的特性。我们选择vqa的理由在于很多研究LLM特性的study里，采用的task都可以被看为是qa或者其变体，所以这里用vqa更合适。其二在于vqa其实包含了多种视觉理解问题，比如有classification，counting，locating等等，通过这个task可以更详尽的探索VLM。同时，相比captioning，VQA更为复杂。

%in this study,我们使用了许多不同的strategies来configure ICEs，比如通过检索相似的图片或者相似的问题作为ICEs，并且在3个各有特色的主流vqa数据集上做了实验，分别是最经典的vqav2,图片文本质量较差的盲人拍摄的vizwiz，需要利用额外知识的okvqa。虽然在实验中我们观察到不同的strategies对不同的数据集有着不同的影响，但是这些diverse observation可以被归结到2个较为本质的原因，分别是1.现在公开的open-flamingo的task recognition能力要强于task learning能力，2.现在的open-flamingo有copy effect.为了进一步的 验证这两个结论，我们也follow之前的NLP studies做了更多的验证实验。


%v2
%近年来，LLM展现了惊人的能力，比如可以通过prompt engineering或者ICL来解决一些新任务，然后研究者就开始使用prompt engineering或者icl来解决问题。但是正如科学家会使用由外向内的方式来理解世界，比如把这个世界作为一个black box，然后做控制变量的实验去观察改变一些input，会得到什么样的output，然后根据这种input-output的反馈来做些猜想，之后再做更多的实验去验证自己的猜想。在研究者使用不同的prompt或者ICL时，他们也发现根据不同的prompt输入进去之后得到的不同反馈，通过这种方式研究者也可以更好的理解大模型。

%相比简单的给一句prompt sentence，ICL是一种更为特f殊的prompt engineering，其prompt为a sequence of ICEs.相比zero-shot的prompt engineering,ICL通常可以取得更好的性能，同时其相比一句话的prompt sentence，更规则也更好控制，所以相对而言更方便研究者去改变ICL的configuration去观察大模型的output，所以NLP里的研究者通过ICL发现了一些大模型的有趣的特性，比如有研究者发现可以把大模型的ICL能力disentangle为Task recognition和Task Learning，也有的研究者发现LLM有copy effect。

%最近，看到LLM的成功，vision-language领域的研究者也开发了有ICL能力的大模型，flamingo和对应的开源版本open-flamingo。但是关于如何在这些模型里找到有效的ICL configuration来解决实际问题的研究还不多，目前只有一个研究captioning的。就vlm领域而言，vqa这个任务也非常重要，其相比captioning也更为复杂。in this study，我们设计了很多strategies来configure ice for solving vqa，一方面探索哪些策略对vqa有效，一方面通过改变icl configuration去更好的understanding现有的vlm的特性。vqa相比caption有两个优势，其一在于nlp中大多数用来研究LLM的方法可以被视为qa，比如sentiment classification可以被认为是在回答what the sentiment of this sentence，所以vqa更为适配，其二在于vqa其实包含了多种视觉理解问题，比如有classification，counting，locating等等，通过这个task可以更详尽的探索VLM。

%为了探索怎么配置ice来更好的解决vqa以及同时探索vlm的特性，我们设计了多种ice strategies，比如xxxxx。

In recent years, Large Language Models (LLMs) have demonstrated remarkable capabilities in solving new tasks through prompt engineering or In-Context Learning (ICL). 
However, despite their success, LLMs still remain opaque and elusive to researchers.
To gain a better understanding of these LLMs, researchers have drawn inspiration from scientists who adopt an outside-in approach to understand the world. 
Similar to the scientists who treat the world as a black box and then conduct controlled experiments to observe the impact of different inputs on outputs, researchers also input different prompts into the LLM to observe the diverse feedback and through these observations, they gain valuable insights about the characteristics of LLMs.
% Taking inspiration from the scientists who adopt an outside-in approach to comprehend the world by treating it as a black box and conducting controlled experiments to observe the impact of varying inputs on outputs, researchers exploring large models have started employing a similar strategy. They find that gaining an understanding of large models is possible by leveraging the diverse feedback by employing different prompts or ICL. 
% To gain a better understanding of these LLMs, researchers have adopted an approach similar to scientists who strive to comprehend the world by treating it as a black box and conducting controlled experiments to observe the impact of varying inputs on outputs. 
% Recently, researchers exploring large models, just like scientists adopt an outside-in approach to comprehend the world, 
% % treating it as a black box and conducting controlled experiments to observe the impact of varying inputs on outputs, 
% have found that the diverse feedback by employing different prompts or ICL enables them to gain a better understanding of large models.

ICL is a specialized form of prompt engineering, utilizing a  sequence of in-context examples (ICEs) as prompts. 
In comparison to the standard single sentence prompt, which is one kind of zero-shot prompt, ICL demonstrates superior performance owing to its few-shot nature, enabling it to encapsulate more information.
% Compared to the standard single sentence prompt, which is one kind of zero-shot prompt, ICL demonstrates superior performance.
However, researchers have discovered significant variations in the performance of LLM in responding to different demonstrations. 
Consequently, many studies in Natural Language Processing (NLP) have been dedicated to investigating how to configure demonstrations to enhance the ICL performance of LLM.
% Many studies in Natural Language Processing (NLP) have explored the effectiveness of in-context configurations. 
Notably, research on ICE selection and ordering has yielded impressive results, underscoring the effectiveness of these demonstration design strategies. 
Meanwhile, as previously mentioned, researchers in NLP have utilized ICL to uncover intriguing characteristics of large models, owing to its superior performance and controllability. 
For example, some researchers have found that the ICL capabilities of Large Language Models can be disentangled into two distinct aspects: task recognition and task learning. Task recognition refers to the model's ability to identify the task at hand and apply pre-trained knowledge, while task learning pertains to its capacity to learn the mapping between input and labels based on provided demonstrations.
% task recognition, the ability to recognize task and apply pre-trained priors, and task learning, the ability to learn the input-label mapping from demonstrations.
% while others have discovered the existence of a copying effect in LMs.

Inspired by the success of Language Models, researchers in the vision-language domain have also developed large models with ICL capabilities, such as Flamingo and its corresponding open-source version, Open-Flamingo. 
However, there is limited research on how to effectively configure demonstrations in these models, both in terms of enhancing the performance of VLM and investigating its characteristics. . 
To the best of our knowledge, currently, only one study has explored demonstration configurations for image captioning. 
Unfortunately, this research still fails to make use of ICL to explore the behaviors and characteristics of VLM. 

In the field of vision-language modeling (VLM), the Visual Question Answering (VQA) task holds equal importance alongside image captioning. Meanwhile, VQA is more suitable for analyzing VLM characteristics through ICL than image captioning for two reasons. 
Firstly, most of the methods used to study LMs in NLP can be considered as question-answering tasks, such as sentiment classification, which can be viewed as answering "what is the sentiment of this sentence?". Therefore, VQA is well-suited for adapting these methods. Secondly, VQA encompasses various visual understanding tasks, including classification, counting, and locating, allowing for a more comprehensive exploration of VLM.


\begin{figure}[htb]
  \centering
  \includegraphics[width=8cm]{figure/tl&tr3.pdf}
  \caption{Task recongnition and task learning.}
  \label{fig:tl&tr}
  % \vspace{-0.2in}
\end{figure}


% and is more complex than captioning. 
% Meanwhile, VQA is more suitable for analyzing VLM characteristics through ICL, which lacks sufficient research attention as well. 

Therefore, in this study, we propose to investigate demonstration configuration in the VQA task with a dual purpose: to explore effective demonstration configuration strategies for enhancing VQA performance and to gain a better understanding of the existing characteristics of VLM by altering the demonstrations.

To investigate the effective configuration of ICEs for VQA, as well as to explore the characteristics of VLM, we design multiple demonstration configuration strategies. These strategies include retrieving demonstrations based on similarity or diversity via images or texts (questions and answers) and reformulating demonstrations after retrieval, for example, mismatching the triplet of (image, question, answer), incorporating instructions and reordering the demonstrations.

% 简单描述一下第3节的method
% To retrieve ICEs, we have two strategies: retrieving examples from the supporting set via images or texts (questions and answers). For image retrieval, two approaches are implemented: retrieving images based on their similarity (I-I-S) and based on their diversity (I-I-D). For questions and answers retrieval, we delved into retrieval based solely on question similarity (Q-Q-S and Q-Q-D) and expanded this to encompass retrieval based on paired question-answer alignment (QA-QA-S). Additionally, a novel approach was explored wherein pseudo answers were utilized for retrieval, termed as A-PA-S.
% Recognizing that the raw retrieval of ICEs might not always yield optimal results, we further manipulated ICEs with an aim to either elevate VQA scores or probe deeper into the characteristics of VLMs. Our suite of manipulations ranged from mismatching the triplet of image, question, and answer, incorporating instructions within the demonstration, to implementing a "strong similarity" method which utilizes visual or linguistic similarity to reorder ices.

% 主要结论，esp tr和tl的假设，第一页会有一张tr，tl示意图
Through experiments involving the retrieval and manipulation of ICEs,our investigation yields three crucial insights.
First, task recognition (TR) holds a more dominant role than task learning (TL) in ICL. TR's emphasis on identifying tasks from ICEs directs models towards potential answer spaces, whereas TL concentrates on learning the input-output mappings directly from the ICEs. 
Second, in VLMs, the textual content in ICEs is paramount compared to visual content. Not only do VLMs exhibit a more pronounced reliance on text quality image quality during the inference phase, but they can also be inadvertently skewed by the textual content within ICEs. Such profound influence culminates in the 'copying effect', a phenomenon where models, rather than processing and reasoning, opt to directly echo answers from contextual texts.
Lastly, similarity-based methods prove generally effective in enhancing VLM performance, while their potency varies depending on the specific dataset and model employed. 
